Spatial Attention Point Network for Deep-learning-based Robust Autonomous Robot Motion Generation

Deep learning provides a powerful framework for automated acquisition of complex robotic motions. However, despite a certain degree of generalization, the need for vast amounts of training data depending on the work-object position is an obstacle to industrial applications. Therefore, a robot motion-generation model that can respond to a variety of work-object positions with a small amount of training data is necessary. In this paper, we propose a method robust to changes in object position by automatically extracting spatial attention points in the image for the robot task and generating motions on the basis of their positions. We demonstrate our method with an LBR iiwa 7R1400 robot arm on a picking task and a pick-and-place task at various positions in various situations. In each task, the spatial attention points are obtained for the work objects that are important to the task. Our method is robust to changes in object position. Further, it is robust to changes in background, lighting, and obstacles that are not important to the task because it only focuses on positions that are important to the task.

==> sections/simulator.tex <==

\subsection{位置変化}

Table.\ref{tab:task_success_rate_simulator_various_position}に
CNNRNN，proposed modelを用いた場合の各点ごとの把持成功率を示す。
CNNRNNの場合，未教示位置（点B，点D）の把持動作成功率は0％であった。
Fig.\ref{fig:Arm_motion_CNNRNN_simulator}に未教示点Bの把持動作の様子を示す。
右の画像につれ時間経過し，4秒間隔で示している。
点Bでなく，近傍の教示点である点Cに向かってアーム手先を近づけ，
把持に失敗しており，未教示位置に汎化されていない。

一方で，proposedを用いた場合，未教示点においても把持成功率が100％であった。
Fig.\ref{fig:Visualizeing_attention_simulator_normal}に，
アーム動作と注視点を可視化した例を示す。
上から順に，Situation1(教示点A)，Situation1(未教示点D)について示す。
右の画像につれ時間経過し，4秒間隔で示している。
画像中の赤い点は，ネットワークのEncoder部から抽出される注視点である。
教示点・未教示点いずれの場合でも，
注視点が対象物近傍に得られており，
タスクに重要な画像特徴量が抽出されており，
対象物の位置変化にロバストとなっている。
なお，画像の中心に空間注意点があるのは，あるチャンネルの特徴マップに特徴が無い場合，
画像の中心に空間注意点が出力されるアルゴリズムになっているためである。

また，この時のモデルの内部状態を可視化するため，
LSTMの内部状態の主成分分析を行った。
Fig.\ref{fig:Attracter_CNNRNN_simulator}，
Fig.\ref{fig:Attracter_attention_simulator}に，
CNNRNN，提案モデルを用いた場合のLSTMの内部状態の主成分分析を行った結果を示す。
%この図はアトラクタと呼ばれ，LSTMの再帰結合層の主成分を無次元の2軸で表したもので，
%各点は各動作の全状態(動作開始時から100 ms毎12秒間の120プロット)を示している。
動作開始時を×，動作終了時を●で示している。
Fig.\ref{fig:Attracter_CNNRNN_simulator}のCNNRNNの場合，
教示点である点A,C,Eについては，
アトラクタが分離されており，
対象物位置に応じて内部状態が異なることが分かる。
しかし，過学習によって未教示点Bと教示点Cの場合でアトラクタが分離されておらず，
未教示点Bの場合に教示点Cと同様な動作をするため，把持失敗していたことが分かる。

一方で，Fig.\ref{fig:Attracter_attention_simulator}の提案モデルの場合，
ブロックの位置に対応し，アトラクタが分離されていることが分かる。
例えば，未教示点Bは教示点AとCの中間に位置するが，
アトラクタも同様に教示点AとCの中間状態となっている。
以上より，対象物の位置変化に対しロバストな動作を獲得できていることを確認できた。
（過学習を防げた）

\begin{table}[htb]
\begin{center}
 \caption{Task success rate}
  \begin{tabular}{|c||c|c|c|c|c|} \hline
    Model\textbackslash Point & A & B & C & D & E \\ \hline
    CNNRNN                    &100\%&      0\%      &100\%&      0\%      &100\% \\ \hline
    Proposed model            &100\%&     100\%     &100\%&     100\%     &100\% \\ \hline 
  \end{tabular}
  \label{tab:task_success_rate_simulator_various_position}
\end{center}
\end{table}

\begin{figure}[htbp]
  \includegraphics[width=8.0cm]{./figs/Arm_motion_CNNRNN_simulator.eps}
  \caption{Arm motion.}
  \label{fig:Arm_motion_CNNRNN_simulator}
\end{figure}

\begin{figure}[htbp]
  \includegraphics[width=8.0cm]{./figs/Visualizing_attention_simulator_normal.eps}
  \caption{Visualizing attention.}
  \label{fig:Visualizeing_attention_simulator_normal}
\end{figure}

\begin{figure}[htbp]%2つに並べて小さくするか
  \includegraphics[width=8.0cm]{./figs/Attracter_CNNRNN_simulator.eps}
  \caption{Attracter.}
  \label{fig:Attracter_CNNRNN_simulator}
\end{figure}

\begin{comment}
\begin{figure}[htbp]
  \includegraphics[width=8.0cm]{./figs/Attracter_attention_simulator.eps}
  \caption{Attracter.}
  \label{fig:Attracter_attention_simulator}
\end{figure}
\end{comment}

%\subsection{照明変化}
\subsection{背景・照明変化，障害物（ロバスト性評価？）}

Table.\ref{tab:task_success_rate_simulator_various_position_bgchange},
Table.\ref{tab:task_success_rate_simulator_various_position_light},
Table.\ref{tab:task_success_rate_simulator_various_position_obstacle}に
それぞれ背景を変えた場合，照明をつけた場合，障害物がある場合における
CNNRNN，提案モデルの把持成功率を示す。
CNNRNNの場合，いずれの場合においても，教示点での把持成功率が下がっており，
タスクに不要である背景や障害物の画像特徴量が抽出されていると考えられる。
なお，背景を変えた場合での未教示点Dの把持成功率が30％となっているが，
これは机の色が変わりブロックの見え方が変わったことで
たまたま把持できるようになったと考えられる。

一方で，提案モデルの場合，いずれの場合においても把持成功率は100％であった。
Fig.\ref{fig:Visualizeing_attention_simulator_change}に，
アーム動作と注視点を可視化した例を示す。
いずれの場合においても，対象物に注視点が得られていることが分かる。
対象物にのみ注視しているため，背景・照明変化や障害物に対しロバストとなっていると
考えられる。

\begin{table}[htb]
\begin{center}
 \caption{Task success rate with background change}
  \begin{tabular}{|c||c|c|c|c|c|} \hline
    Model\textbackslash Point & A & B & C & D & E \\ \hline
    CNNRNN                    &100\%&      0\%      &90\%&      30\%      &100\% \\ \hline
    Proposed model            &100\%&     100\%     &100\%&     100\%     &100\% \\ \hline 
  \end{tabular}
  \label{tab:task_success_rate_simulator_various_position_bgchange}
\end{center}
\end{table}

\begin{table}[htb]
\begin{center}
 \caption{Task success rate with light change}
  \begin{tabular}{|c||c|c|c|c|c|} \hline
    Model\textbackslash Point & A & B & C & D & E \\ \hline
    CNNRNN                    &100\%&      0\%      &90\%&      0\%      &90\% \\ \hline
    Proposed model            &100\%&     100\%     &100\%&     100\%     &100\% \\ \hline 
  \end{tabular}
  \label{tab:task_success_rate_simulator_various_position_light}
\end{center}
\end{table}

\begin{table}[htb]
\begin{center}
 \caption{Task success rate with obstacle}
  \begin{tabular}{|c||c|c|c|c|c|} \hline
    Model\textbackslash Point & A & B & C & D & E \\ \hline
    CNNRNN                    &50\%&      0\%      &0\%&      0\%      &70\% \\ \hline
    Proposed model            &100\%&     100\%     &100\%&     100\%     &100\% \\ \hline 
  \end{tabular}
  \label{tab:task_success_rate_simulator_various_position_obstacle}
\end{center}
\end{table}

\begin{figure}[htbp]
  \includegraphics[width=8.0cm]{./figs/Visualizing_attention_simulator_change.eps}
  \caption{Visualizing attention.}
  \label{fig:Visualizeing_attention_simulator_change}
\end{figure}




\begin{comment}
\begin{figure}[htbp]
  \includegraphics[width=8.0cm]{./figs/Visualizing_attention_simulator_shadow.eps}
  \caption{Visualizing attention.}
  \label{fig:Visualizeing_attention_simulator_shadow}
\end{figure}

\begin{figure}[htbp]
  \includegraphics[width=8.0cm]{./figs/Visualizing_attention_simulator_bg.eps}
  \caption{Visualizing attention.}
  \label{fig:Visualizeing_attention_simulator_bg}
\end{figure}

\begin{figure}[htbp]
  \includegraphics[width=8.0cm]{./figs/Visualizing_attention_simulator_obstacle.eps}
  \caption{Visualizing attention.}
  \label{fig:Visualizeing_attention_simulator_obstacle}
\end{figure}
\end{comment}
%\subsection{障害物}
%\subsection{背景変化}
